DELVE-ing into the Jet: a thin stellar stream on a retrograde orbit at 30 kpc

We perform a detailed photometric and astrometric analysis of stars in the Jet stream using data from the first data release of the DECam Local Volume Exploration Survey (DELVE) DR1 and \emph{Gaia} EDR3. We discover that the stream extends over $\sim 29 ^{\circ}$ on the sky (increasing the known length by $18^{\circ}$), which is comparable to the kinematically cold Phoenix, ATLAS, and GD-1 streams. Using blue horizontal branch stars, we resolve a distance gradient along the Jet stream of 0.2 kpc/deg, with distances ranging from $D_\odot \sim 27-34$ kpc. We use natural splines to simultaneously fit the stream track, width, and intensity to quantitatively characterize density variations in the Jet stream, including a large gap, and identify substructure off the main track of the stream. Furthermore, we report the first measurement of the proper motion of the Jet stream and find that it is well-aligned with the stream track suggesting the stream has likely not been significantly perturbed perpendicular to the line of sight. Finally, we fit the stream with a dynamical model and find that the stream is on a retrograde orbit, and is well fit by a gravitational potential including the Milky Way and Large Magellanic Cloud. These results indicate the Jet stream is an excellent candidate for future studies with deeper photometry, astrometry, and spectroscopy to study the potential of the Milky Way and probe perturbations from baryonic and dark matter substructure.

==> table_results_eye.tex <==
\begin{deluxetable}{l ccccc }[hb!]
\tablecolumns{13}
\tablewidth{0pt}
\tabletypesize{\scriptsize}
\tablecaption{ \eyecaption \label{tab:results_eye}}
\tablehead{ & $\mu_{\rm \alpha} cos \delta$ & $\mu_{\rm \delta}$ & $\mu_{\rm \phi_1}$ & $\mu_{\rm \phi_2}$ \\
 & (mas/yr) & (mas/yr) & (mas/yr) & (mas/yr)}
\startdata
Aliqa Uma       &  0.3 & -0.6 &  1.0 & -0.2 \\
ATLAS           & -0.1 & -1.0 &  1.6 & -0.2 \\
Chenab          &  0.3 & -2.4 &  1.0 & -0.5 \\
Elqui           &  0.1 & -0.4 &  0.6 &  0.0 \\
Indus           &  3.5 & -5.4 & -3.8 &  0.1 \\
Jhelum          &  6.9 & -5.8 & -6.0 & -0.8 \\
Phoenix         &  2.8 & -0.1 & -1.9 & -0.4 \\
Tucana III      & -0.1 & -1.7 &  1.1 &  0.0 \\
Turranburra     &  0.4 & -0.9 &  0.8 & -0.3 \\
[+0.5em]\tableline\\[-1em]
Ravi            &  0.2 & -1.6 & 0.5 &  -0.1 \\
Turbio          &  2.3 &  2.0 & -3.8 & -0.3 \\
Wambelong       &  2.0 & -0.1 & -0.8 & -0.9 \\
Willka Yaku     &  1.1 &  0.3 &  -0.9 &  0.0 \\
Molonglo        & \ldots &  \ldots & \ldots &  \ldots \\
\enddata
% {\footnotesize \tablecomments{ \eyecomments }}
\end{deluxetable}

